Binary Decision Diagrams: from Tree Compaction to Sampling

Any Boolean function corresponds with a complete full binary decision tree. This tree can in turn be represented in a maximally compact form as a direct acyclic graph where common subtrees are factored and shared, keeping only one copy of each unique subtree. This yields the celebrated and widely used structure called reduced ordered binary decision diagram (ROBDD). We propose to revisit the classical compaction process to give a new way of enumerating ROBDDs of a given size without considering fully expanded trees and the compaction step. Our method also provides an unranking procedure for the set of ROBDDs. As a by-product we get a random uniform and exhaustive sampler for ROBDDs for a given number of variables and size.

==> sections/concl.tex <==

As a conclusion a special highlight of the method we used must be given.
First, by adapting the combinatorial specification, thus the unranking algorithm,
we manage to select the subclass of Boolean functions whose variables are all
essential. Their study is exhibited in Appendix~\ref{app:essential}.
Furthermore, our combinatorial analysis of the compaction process underlying \BDDs~can
be generalized to study other kind of structures resulting of some compaction process.
In the last part of the Appendices (see~\ref{sec:QRBDD} and~\ref{sec:ZBDD})
we underline this fact by
exhibiting the same kind of results for other kinds of decision diagrams, usually called
\textsc{qbdd}s or \textsc{zbdd}s.

Finally in the same vein of study, a combinatorially
analysis of the compaction of tries would be a possible further work.
Recall that tries, or digital trees are very common data structures,
and their tree-structure is now well known, cf. e.g.~\cite{CFV01}.


 
